VividDream: Generating 3D Scene with Ambient Dynamics

We introduce VividDream, a method for generating explorable 4D scenes with ambient dynamics from a single input image or text prompt. VividDream first expands an input image into a static 3D point cloud through iterative inpainting and geometry merging. An ensemble of animated videos is then generated using video diffusion models with quality refinement techniques and conditioned on renderings of the static 3D scene from the sampled camera trajectories. We then optimize a canonical 4D scene representation using an animated video ensemble, with per-video motion embeddings and visibility masks to mitigate inconsistencies. The resulting 4D scene enables free-view exploration of a 3D scene with plausible ambient scene dynamics. Experiments demonstrate that VividDream can provide human viewers with compelling 4D experiences generated based on diverse real images and text prompts.

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/macros.tex <==
% Macros - Jia-Bin Huang (jbhuang0604@gmail.com)

% \renewcommand{\baselinestretch}{0.991}       % for squeezing the draft into the page limit, do not use

% For the unsure command.
\usepackage{soul}
\usepackage{svg}

% \usepackage[accsupp]{axessibility} % Improves PDF readability for those with disabilities.

% \usepackage[final]{changes}

\newcommand{\tae}[1]{{\textcolor{blue}{Tae: #1}}}

% =========================================
% Useful macros
% =========================================

% Latin abbreviations
\def\etal{et~al.}			  % and others, and co-workers
\def\eg{e.g.,~}               % for example
\def\ie{i.e.,~}               % that is, in other words
\def\etc{etc}                 % and other things, and so forth
\def\cf{cf.~}                 % compare
\def\viz{viz.~}               % namely, precisely
\def\vs{vs.~}                 % against

\def\naive{na{\"i}ve\xspace}
\def\Naive{Na{\"i}ve\xspace}
\def\naively{na{\"i}vely\xspace}
\def\Naively{Na{\"i}vely\xspace}

% Math related
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\minimize}{minimize}

\DeclareMathAlphabet{\altmathcal}{OMS}{cmsy}{m}{n}
\DeclareMathAlphabet{\mathbfit}{OT1}{ptm}{bx}{it}

% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin

\newlength\secmargin
\newlength\figcapmargin
\newlength\tabcapmargin

\setlength{\secmargin}{0.0mm}
\setlength{\paramargin}{0.0mm}
\setlength{\figmargin}{0.0mm}
\setlength{\figcapmargin}{-0mm}
\setlength{\tabcapmargin}{0.0mm}

\setlength{\fboxsep}{0pt}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\changed}{\textcolor{black}} 

% minipage
\newcommand{\mpage}[2]
{
\begin{minipage}{#1\linewidth}\centering
#2
\end{minipage}
}

\newcommand{\mfigure}[2]
{
\includegraphics[width=#1\linewidth]{#2}
}

\newcommand{\myparagraph}[1]
{
\vspace{-1.5pt}\paragraph{#1}
}

% References for figures, tables, equations, and sections
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}} 
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}

% Comments
\long\def\ignorethis#1{}
%\newcommand {\jiabin}[1]{{\color{cyan}\textbf{Jia-Bin: }#1}\normalfont}
%\newcommand {\junyan}[1]{{\color{red}\textbf{Jun-Yan: }#1}\normalfont}
\newcommand {\taesung}[1]{{\color{magenta}#1}\normalfont}
%\newcommand {\songwei}[1]{{\color{blue}\textbf{Songwei: }#1}\normalfont}
\newcommand {\jiabin}[1]{}
\newcommand {\junyan}[1]{}
%\newcommand {\taesung}[1]{}
\newcommand {\songwei}[1]{}
\newcommand {\new}[1]{{\color{magenta}#1}\normalfont}

%\newcommand {\todo}{{\textbf{\color{red}[TO-DO]\_}}}
\def\newtext#1{\textcolor{blue}{#1}}
\def\modtext#1{\textcolor{red}{#1}}
%\newcommand{\note}[1]{{\it\color{blue} #1}}

%\newcommand{\unsure}[1]{{\sethlcolor{yellow}\hl{#1}}}

\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
}

% subfigures with automatic width
\newbox\jsavebox%
\newcommand{\jsubfig}[2]{%
	\sbox\jsavebox{#1}%
	\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
	}

%%%%%%%%%%%%%%%%	
%% \providelength command that will define a new length if not already defined, but
%% also checks whether the command passed as argument has been defined with
%% \newlength, in order to issue an error message if you try to use, say,
%% \providelength{\textit}
\makeatletter
\newcommand{\providelength}[1]{%
  \@ifundefined{\expandafter\@gobble\string#1}
   {% if #1 is undefined, do \newlength
    \typeout{\string\providelength: making new length \string#1}%
    \newlength{#1}%
   }
   {% else check whether #1 is actually a length
    \sdaau@checkforlength{#1}%
   }%
}

\newcommand{\sdaau@checkforlength}[1]{%
  % get the first five characters from \meaning#1
  \edef\sdaau@temp{\expandafter\sdaau@getfive\meaning#1TTTTT$}%
  % compare with the string "\skip"
  \ifx\sdaau@temp\sdaau@skipstring
    \typeout{\string\providelength: \string#1 already a length}%
  \else
    \@latex@error
      {\string#1 illegal in \string\providelength}
      {\string#1 is defined, but not with \string\newlength}%
  \fi
}
\def\sdaau@getfive#1#2#3#4#5#6${#1#2#3#4#5}
\edef\sdaau@skipstring{\string\skip}
\makeatother
%%%%%%%%%%%%%%%%%%%%%



==> setup/package.tex <==
% Fix "undefined control sequence \Everyshipout".
% \usepackage{everyshi}

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
% \usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{caption}
\usepackage{lscape}                                         % Useful for wide tables or figures.
\usepackage{wrapfig}
\usepackage{pgfplots}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0mm}

% Math
% \usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
% \usepackage{times}
% \usepackage{mathptmx}
% \usepackage{mathtools}
% \usepackage{amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}

% Comments
% \usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
\usepackage{xspace}
% \usepackage[table]{xcolor}
\usepackage{grfext}
\PrependGraphicsExtensions*{.jpg,.png,.PNG}
\definecolor{firebrick}{HTML}{d48265}
\definecolor{lightfirebrick}{HTML}{c23531}
% \definecolor{firebrick}{rgb}{0.59, 0.1, 0.1}
% \definecolor{lightfirebrick}{rgb}{0.95, 0.33, 0.33}
\definecolor{grayblue}{HTML}{61a0a8}
\definecolor{lightgrayblue}{HTML}{2f4554}
\definecolor{turquoise}{rgb}{0., 0.4, 0.7}
\definecolor{lightturquoise}{rgb}{0.4, 0.8, 0.96}
\definecolor{goldyellow}{rgb}{0.964, 0.886, 0.4}
\definecolor{lightorange}{HTML}{C27000}
\definecolor{darkorange}{HTML}{D3A171}
% \definecolor{lightorange}{rgb}{1., 0.9, 0.3}
\definecolor{lightgreen}{HTML}{61a0a8}
\definecolor{darkgreen}{HTML}{749f83}


\usepackage{textcomp,gensymb}
% \usepackage{emoji}
\usepackage{tikz}
% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


% Hyperlinks
%\usepackage{url}  % Hyphenation of URLs.
% \usepackage[hyphens]{url}
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
% \usepackage{xspace}
% \usepackage[table]{xcolor}
% \usepackage{setspace}
% \usepackage{grfext}
% \PrependGraphicsExtensions*{.jpg,.png,.PNG}

% \usepackage{gensymb}
% \usepackage{emoji}

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese

% \usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

% vertical rule
\newcommand{\rulesep}{\unskip\ \vrule\ }

% footnote
\usepackage[symbol]{footmisc}

% table
\usepackage{soul} % \ul
\usepackage{multirow}

\usepackage{pifont}
